Efficient Top-K Retrieval in Online Social Tagging Networks

We consider in this paper top-k query answering in social tagging systems, also known as folksonomies. This problem requires a significant departure from existing, socially agnostic techniques. In a network-aware context, one can (and should) exploit the social links, which can indicate how users relate to the seeker and how much weight their tagging actions should have in the result build-up. We propose an algorithm that has the potential to scale to current applications. While the problem has already been considered in previous literature, this was done either under strong simplifying assumptions or under choices that cannot scale to even moderate-size real world applications. We first consider a key aspect of the problem, which is accessing the closest or most relevant users for a given seeker. We describe how this can be done on the fly (without any pre-computations) for several possible choices - arguably the most natural ones - of proximity computation in a user network. Based on this, our top-k algorithm is sound and complete, while addressing the scalability issues of the existing ones. Importantly, our technique is instance optimal in the case when the search relies exclusively on the social weight of tagging actions. To further reduce response times, we then consider directions for efficiency by approximation. Extensive experiments on real world data show that our techniques can drastically improve the response time, without sacrificing precision.

==> related.tex <==
\section{Related Work}\label{sec:related}

Lately, the topic of search in a social setting has garnered increased attention. Studies and models of personalization of social tagging sites can be found in~\cite{Wang10,Heymann08,Dou07,Xu08}. Other studies have found that including social knowledge in scoring models can improve search and recommendation algorithms. In~\cite{Carmel09}, personalization based on a similarity network is shown to outperform other personalization approaches and the non-personalized social search. A study on a last.fm dataset in~\cite{Konstas09} has found that incorporating social knowledge in a graph model system improves the retrieval recall of music track recommendation algorithms.

The scoring model used in~\cite{Schenkel08} is revisited in~\cite{Yin10}, in which a textual relevance part and a social influence part are combined for the scoring of items, the social influence being calculated as the inverse of the shortest path between the seeker and the document publishers.

A more general approach for social search is given in~\cite{Amer-Yahia09,Amer-Yahia09SS}, in which a algebraic framework for graph manipulation is established for formalizing information discovery in social content sites.
